Hierarchical Experience-informed Navigation for Multi-modal Quadrupedal Rebar Grid Traversal

This study focuses on a layered, experience-based, multi-modal contact planning framework for agile quadrupedal locomotion over a constrained rebar environment. To this end, our hierarchical planner incorporates locomotion-specific modules into the high-level contact sequence planner and solves kinodynamically-aware trajectory optimization as the low-level motion planner. Through quantitative analysis of the experience accumulation process and experimental validation of the kinodynamic feasibility of the generated locomotion trajectories, we demonstrate that the experience planning heuristic offers an effective way of providing candidate footholds for a legged contact planner. Additionally, we introduce a guiding torso path heuristic at the global planning level to enhance the navigation success rate in the presence of environmental obstacles. Our results indicate that the torso-path guided experience accumulation requires significantly fewer offline trials to successfully reach the goal compared to regular experience accumulation. Finally, our planning framework is validated in both dynamics simulations and real hardware implementations on a quadrupedal robot provided by Skymul Inc.

==> 10SentenceSummary.tex <==
TODO: Create the 10 sentence summary of what the paper should be about (can be up to 20, but the idea is to keep it concise as well as to use language that is not overly technical). This summary should be a guide towards writing the overall paper. The more intelligible it is to non-technical people, the better (I always ask myself: “Could a non-engineer understand it, or get the gist?”, maybe with one or two technical nuggets of additional information).


10 Sentence Summary:
Legged robots have showcased impressive locomotion feats, ranging from running to jumping to parkour. A key aspect to generating trajectories for legged locomotion is how to plan contacts throughout the environment that move the robot to its goal. State-of-the-art footstep planning largely relies on heuristic or approximate methods in order to formulate tractable problems and obtain low run-times. As a result, these footstep planning approaches lack any sort of performance or safety guarantee, and instead rely on emergent characteristics of these planning methods for success and robustness.

Multi-modal planning on constrained manifolds is an approach previously applied to robotic manipulation tasks that yields probabilistic completeness guarantees: if a feasible solution exists to a motion planning problem, then it will be found given enough computing time. In this work, we adapt this multi-modal framework to quadrupedal systems as a first use case of this framework on legged locomotion tasks. To accomplish this, we also embed quadrupedal dynamics into this multi-modal framework, which has previously only been used in conjunction with kinematic constraints. In doing so, we are able to provide formal task completion guarantees for quadrupedal navigation along these rebar grids. Additionally, we employ adaptive sampling methods by leveraging additional constraints such as given contact sequences and center-of-mass trajectories that restrict the otherwise computationally-expensive branching factor of such high-dimensional systems.

We verify such performance guarantees in a simulated rebar-grid environment in which the quadruped is constrained to traversing along the physical rebar.

==> text_files/LimitationsAndFutureWork.tex <==
\section{Limitations And Future Work} \label{sec:limitations}


==> text_files/MultiModalNavigation.tex <==
\section{Multi-modal Navigation} \label{sec:mmn}
In this section, we cover the higher torso-planning level of the hierarchical navigation framework. This framework decomposition leverages a common model in legged navigation in which at the top level, a coarse plan from start to goal is generated using only the torso for the robot model. This suggested torso path is then passed to the lower level of the navigation framework (here, the multi-modal contact planner) in which a kinodynamically-aware legged robot model is used to generate a whole-body path from start to goal. We detail the torso planner used in this work, but it is important to note that this hierarchical navigation framework is generalizable enough to accept any torso planner that provides a sequence of torso poses from start to goal.

For this work, we formulate the torso path planning task as an additional graph search problem in which A* is employed. The 6-DOF torso state is projected down onto the 2D rebar grid, yielding a state space of $\mathbf{x} = [x_{\rm torso}, y_{\rm torso}]$. The environment of the rebar grid is discretized so that state space tuples align with the intersections on the rebar grid. 

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/torso_plan_grid.jpg}
    \caption{Rebar grid for torso path planning. Blue dots along the grid intersections represent state space tuples used in the state space search. Red represents obstacles and orange represents inflated obstacles. Green and red dots represent the start and goal nodes respectively, and the purple line represents the resulting torso path. }
    \label{fig:torso_plan_grid}
\end{figure}
\end{comment}

Transitions between adjacent cells are added to the state space graph, and the edge cost for these transitions is
%
\begin{equation}
    \Delta c(\mathbf{x}_1, \mathbf{x}_2) = d(\mathbf{x}_1, \mathbf{x}_2) + w_{\rm obst}(\mathbf{x}_1, \mathbf{x}_2)
\end{equation}
%
where $d(\mathbf{x}_1, \mathbf{x}_2)$ is the Euclidean distance between tuples $\mathbf{x}_1$ and $\mathbf{x}_2$ and $w_{\rm obst}$ is a weight based on the proximity of tuples $\mathbf{x}_1$ and $\mathbf{x}_2$ to the set of environment obstacles $O$ as well as the set of inflated obstacles $O_{\rm infl}$:
%
\begin{equation}
    w_{\rm obst}(\mathbf{x}_1, \mathbf{x}_2) = \begin{cases}
                                            100, & \mathbf{x}_1 \in{} O \text{ or } \mathbf{x}_2 \in{} O \\
                                            25, & \mathbf{x}_1 \in{} O_{\rm infl} \text{ or } \mathbf{x}_2 \in{} O_{\rm infl} \\
                                            0, & \text{else}
                                           \end{cases}
\end{equation}

A simple search heuristic of
\begin{equation}
    g(\mathbf{x}) = d(\mathbf{x}, \mathbf{x}_{\rm goal})
\end{equation}
where $d(\mathbf{x}, \mathbf{x}_{\rm goal})$ is the Euclidean distance between tuples $\mathbf{x}$ and $\mathbf{x}_{\rm goal}$ is used to ensure an admissible search heuristic and optimal torso paths.
